Neural Graphics Texture Compression Supporting Random Access

Advances in rendering have led to tremendous growth in texture assets, including resolution, complexity, and novel textures components, but this growth in data volume has not been matched by advances in its compression. Meanwhile Neural Image Compression (NIC) has advanced significantly and shown promising results, but the proposed methods cannot be directly adapted to neural texture compression. First, texture compression requires on-demand and real-time decoding with random access during parallel rendering (e.g. block texture decompression on GPUs). Additionally, NIC does not support multi-resolution reconstruction (mip-levels), nor does it have the ability to efficiently jointly compress different sets of texture channels. In this work, we introduce a novel approach to texture set compression that integrates traditional GPU texture representation and NIC techniques, designed to enable random access and support many-channel texture sets. To achieve this goal, we propose an asymmetric auto-encoder framework that employs a convolutional encoder to capture detailed information in a bottleneck-latent space, and at decoder side we utilize a fully connected network, whose inputs are sampled latent features plus positional information, for a given texture coordinate and mip level. This latent data is defined to enable simplified access to multi-resolution data by simply changing the scanning strides. Experimental results demonstrate that this approach provides much better results than conventional texture compression, and significant improvement over the latest method using neural networks.

==> sections/introduction_old.tex <==
\begin{figure*}
     \begin{subfigure}[b]{0.6\textwidth}
         \centering
         \includegraphics[width=1\textwidth]{eccv-2024//Figs/cntc_scheme.pdf}
         \caption{}
         \label{fig:main_arch}
     \end{subfigure}
     \hspace{0.1cm}
     \begin{subfigure}[b]{0.35\textwidth}
         \centering
         \includegraphics[width=1\textwidth]{eccv-2024//Figs/ours_ntc_astc_2k_rd.pdf}
         \caption{}
         \label{fig:rd_curve}
     \end{subfigure}
     \vspace{-0.25cm}
        \caption{(a) Overview of our neural texture compression (b) Rate-Distortion (RD) curve.  Our method significantly outperforms the state-of-the-art texture compression method, NTC~\cite{Vaidyanathan2023}, with a 40.8\% in the BD-rate saving.}
        % Vertical axis: PSNR scores of different methods. 
        % The horizontal axis is bits per pixel per channel storage cost.
        \label{fig:archs}
    \vspace{-0.3cm}
\end{figure*}

The rapid growth of graphics and gaming industries hinges on new technologies that create increasingly photorealistic scenes. However, achieving realism necessitates vast amounts of data, which can impact download times, rendering speed, and local storage. 

Most of this data is composed of graphics textures, which are collections of 2D arrays with information about how a 3D object's surface appearance should change according to lighting and viewing position~\cite{shirley2009fund,hughes2013intro}. The amount of data has been reduced with some widely used texture compression methods, but those are comparatively limited and inefficient, and the development of better compression has been very slow due to several technical difficulties.

Textures often appear magnified and can have large sizes with multiple components, organized in a multi-resolution mipmap pyramid (e.g., 16 × 8K × 8K). However, only a small fraction of this data is necessary for a specific scene view. Efficient texture compression methods are essential to decompress only the required components. Additionally, the compression must support fast and asynchronous parallelized execution, allowing each rendering thread to independently access the necessary values for its tasks at the required position and resolution. 

This requirement alone eliminates several of the most efficient techniques used for compressing 2D images and videos, that exploit wide scale dependencies, statistical consistency, and serialized entropy coding, and that consequently cannot be independently decompressed. 

Another complication is that rendering is fully programmable, enabling the creation of an increasing variety of texture components. Thus, the design of methods that can optimally compress all new texture component types cannot be done manually, and must be automated via learning-based techniques.

Compression methods using neural networks have been proposed for images and video, and shown to be competitive to conventional methods. Unfortunately, those codec architectures are also not designed and cannot be easily modified to support random access and other rendering requirements. This paper addresses this problem by proposing new learning-based methods and neural-network architectures specifically designed for texture compression and rendering.

Photorealistic rendering aims to create digital images that closely resemble real-world photographs. Achieving this level of realism heavily relies on texturing, which endows surfaces with realistic characteristics like roughness, smoothness, reflectivity, and intricate patterns. By adding depth and tactile qualities to objects, texturing enhances their overall believability. It allows faithful replication of various materials such as wood, metal, fabric, glass, or concrete, significantly contributing to the overall realism of rendered scenes. However, texturing comes with a trade-off: it requires storing substantial amounts of data corresponding to different materials.

In the realm of computer graphics, mipmaps play a crucial role in texture resampling. Imagine them as a well-organized image pyramid, meticulously designed for efficient texture filtering. Each mip level represents a filtered version of the texture, corresponding to a specific image pixel-to-texture pixel ratio. Since mipmaps are pre-allocated, additional storage space is necessary to fully leverage their benefits \cite{MIPMAP_wk}. 

Compared to digital image compression, texture compression present additional challenges. While digital image compression focuses on compressing an entire image at a fixed resolution, graphics textures may need to be rendered at different resolutions and mip levels. Moreover, only a portion of the texture might require rendering, necessitating random access to the texture data at any resolution and position. Unlike neural image compression, which handles a fixed number of color channels (e.g., 3 channels for RGB or YUV), texture compression faces unique complexities. %\hoang{there are 2 things: image compression and reconstruction: I don't see a clear comparison with them in this paragraph;}

\section{Motivation}
\label{sec:motivation}
Conventional texture compression achieves random access by employing block-wise vector quantization. These techniques often leverage both spatial and cross-channel correlations. However, their limitation lies in the fact that they can only compress textures with up to ``four channels''. In contrast, modern renderers commonly utilize a broader range of material properties, including color channels as well as other channels for normal maps, height maps, ambient occlusion, glossiness, roughness, and other information related to the Bidirectional Reflectance Distribution Function (BRDF).

These channels exhibit significant correlation within the texture set. This correlation arises from a combination of factors, including physical material properties, geometric features, and artistic layering during material authoring~\cite{Hill2020}. For instance, consider Figure~\ref{fig:texture_set_brick}, where a texture set related to a brick wall pattern includes color channels as well as other channels for normal map, ARM (ambient occlusion, roughness, metalness) map, and displacement map. 

Furthermore, in computer graphics, for efficient rendering textures are stored at different resolutions, commonly referred to as mipmaps. 
As shown by~\cite{Bartlomiej2021} there are significant redundancies at different scales. 

In their pioneering work, Vaidyanathan et al.~\cite{Vaidyanathan2023}, introduced a novel neural texture compression scheme. Their approach exploits spatial redundancies across all channels of a texture set and across different mip levels. They achieved this by compressing the entire texture set, including all channels and mip levels simultaneously. Their autodecoder framework~\cite{Park2019-nu} utilizes a pair of feature pyramids, referred to as Girds, to represent the texture set throughout all mip levels. Each pyramid level is responsible for reconstructing texels at one or more mip levels, and features stored at a particular pyramid level can be shared across multiple mip levels. This innovative method significantly advances texture compression efficiency and quality in texture representation.

In our analysis, we identified redundancy within the feature pyramids, which adversely affected compression performance. Particularly, as texture resolution increased, this redundancy became more pronounced. 
Figure~\ref{fig:cka} illustrates centered kernel alignment (CKA)~\cite{Kornblith2019-qn} across different levels of the feature pyramid $F^l_0$ and $F^l_1$. 
$\mathrm{CKA}_i(k,l)$ represents the similarity between features stored at pyramid levels $k$ and $l$ of a grid $F_i$, %i.e., $G^k_i$ and $G^l_i$ derived by NTC \cite{Vaidyanathan2023}. 
specifically $F^k_i$ and $F^l_i$ derived using the NTC method by~\cite{Vaidyanathan2023}. 

\begin{figure}[t]
\centering
    \begin{subfigure}[b]{0.2\textwidth}
         \centering         
         \includegraphics[width=1\textwidth]{eccv-2024/Figs/cka_grid_0_nvidia.pdf}         
         \caption{$\mathrm{CKA}_0$}
         \label{}
    \end{subfigure}
    \hspace{1cm}
    \begin{subfigure}[b]{0.2\textwidth}
         \centering
         \includegraphics[width=1\textwidth]{eccv-2024//Figs/cka_grid_1_nvidia.pdf}
         \caption{$\mathrm{CKA}_1$}
         \label{}
    \end{subfigure}
    \vspace{-0.2cm}
    \caption{Centered kernel alignment (CKA) of features stored at pyramid levels $k$ and $l$ of the feature pyramid $F_i$, i.e., $F^k_i$ and $F^l_i$, evaluated on “Ceramic roof 01” texture set,
retrieved from \url{https://polyhaven.com/}.}%\hoang{each square is too big, this can be much smaller}}
    \label{fig:cka}
    \vspace{-0.2cm}
\end{figure}


In our investigation (Figure~\ref{fig:cka}), we have observed substantial similarity across various levels of the feature pyramids, which suggests the presence of redundant data. To tackle this issue, we propose an innovative neural texture compression method based on an asymmetric autoencoder framework. The key contributions of our approach are as follows (see Figure~\ref{fig:main_arch}):
\begin{enumerate}
    \item Asymmetric autoencoder framework: Our ``Global transformer'' processes a texture set and generates representations that capture spatial-channel-resolution redundancy. The ``texture synthesizer'' then samples from these representations to reconstruct texels at specific positions and mip levels.%\hoang{"compress" this to be a single sentence = single contribution}
    \item Grid Constructor: The global transformer exclusively operates on the texture set at the highest resolution (mip level 0) and maps it into a pair of single-resolution representations. These pair of representations capture high and low frequency features of the texture set and serve as the representation across all mip levels.
    \item Grid sampler: To facilitate texel reconstruction from different mip levels, we sample the features stored in the representations using varying strides.
\end{enumerate}
By leveraging redundancies across pixels, different channels and mip levels, our method enhances texture compression while maintaining quality. 

\begin{figure}
\captionsetup[subfigure]{labelformat=empty}
\centering
    \begin{subfigure}[b]{0.15\textwidth}
         \centering         
         \includegraphics[width=1\textwidth]{eccv-2024/Figs/Diffuse_1k.png}         
         \caption{\scriptsize diffuse}
         \label{}
    \end{subfigure}
    \hspace{0.5cm}
    \begin{subfigure}[b]{0.15\textwidth}
         \centering
         \includegraphics[width=1\textwidth]{eccv-2024//Figs/nor_gl_1k.png}
         \caption{\scriptsize normal}
         \label{}
    \end{subfigure}
    \hspace{0.5cm}
    \begin{subfigure}[b]{0.15\textwidth}
         \centering
         \includegraphics[width=1\textwidth]{eccv-2024//Figs/Displacement_1k.png}         
         \caption{\scriptsize displacement}
         \label{}
    \end{subfigure}
    \hspace{0.5cm}
    \begin{subfigure}[b]{0.15\textwidth}
         \centering
        \includegraphics[width=1\textwidth]{eccv-2024//Figs/arm_1k.png}
         \caption{\scriptsize ARM}
         \label{}
    \end{subfigure}
    \vspace{-0.3cm}
    \caption{An example of texture set consisting of a diffuse map, normal map, an ARM (ambient occlusion, roughness, metalness) map, and a displacement map, for a brick wall pattern retrieved from  \url{https://polyhaven.com}.}
    \label{fig:texture_set_brick}
    \vspace{-0.3cm}
\end{figure}

==> supplemantary/errata.tex <==

Presented below is the rectification for Figure~5. Regrettably, an error exists in Figure~5 within Section~5.2. The curve associated with our method has been inaccurately plotted. For the corrected curve related to our method, kindly consider Figure~\ref{fig:rd_curve_corrected}. 

\begin{figure}[h!]
    \centering
     \begin{subfigure}[b]{0.47\textwidth}
         \centering
         \includegraphics[width=1\textwidth]{Figs/ours_ntc_astc_2k_rd_corrected.pdf}
         % \caption{}
         \label{fig:rd_curve_psnr}
     \end{subfigure}
     \hspace{-0cm}
     \begin{subfigure}[b]{0.485\textwidth}
         \centering
         \includegraphics[width=1\textwidth]{Figs/ours_ntc_astc_2k_rd_ssim_corrected.pdf}
         % \caption{}
         \label{fig:rd_curve_ssim}
     \end{subfigure}
     % \vspace{-0.2in}
    \caption{Comparison with the state-of-the-art method NTC~\cite{Vaidyanathan2023}.}
    \label{fig:rd_curve_corrected}
\end{figure}

